Sensitivity and Reliability in Incomplete Networks: Centrality Metrics to Community Scoring Functions

Network analysis is an important tool in understanding the behavior of complex systems of interacting entities. However, due to the limitations of data gathering technologies, some interactions might be missing from the network model. This is a ubiquitous problem in all domains that use network analysis, from social networks to hyper-linked web networks to biological networks. Consequently, an important question in analyzing networks is to understand how increasing the noise level (i.e. percentage of missing edges) affects different network parameters. In this paper we evaluate the effect of noise on community scoring and centrality-based parameters with respect to two different aspects of network analysis: (i) sensitivity, that is how the parameter value changes as edges are removed and (ii) reliability in the context of message spreading, that is how the time taken to broadcast a message changes as edges are removed. Our experiments on synthetic and real-world networks and three different noise models demonstrate that for both the aspects over all networks and all noise models, permanence qualifies as the most effective metric. For the sensitivity experiments closeness centrality is a close second. For the message spreading experiments, closeness and betweenness centrality based initiator selection closely competes with permanence. This is because permanence has a dual characteristic where the cumulative permanence over all vertices is sensitive to noise but the ids of the top-rank vertices, which are used to find seeds during message spreading remain relatively stable under noise.

==> definition.tex <==
\section{Permanence as a centrality metric}\label{definition}

We first provide a brief introduction to permanence. Permanence was introduced in ~\cite{chakraborty2014permanence} as a vertex-centric metric for evaluating the quality of communities in a network. If the community structure is known, permanence is defined for each vertex  as follows;
$P(v) = [\frac{I(v)}{E_{max}(v)} \times \frac{1}{D(v)} - (1 - c_{in}(v)) ]$ \\
where $I(v)$ is the number of neighbours of $v$ in its community, $E_{max}(v)$ is the maximum number of connections of $v$ in its neighbouring community, $D(v)$ is the degree of $v$ and $c_{in}(v)$ is the internal clustering coefficient of the internal nodes of $v$ in the community. Permanence tries to formulate the ``pull'' experienced by a vertex $v$ from its external neighbors, i.e., neighbors residing in communities different from that of $v$. If this pull is low (low $E_{max}(v)$) and the internal neighbors in the community of $v$ are tightly connected (high $c_{in}(v)$) then there is a high probability that $v$ is very "`stable'' in its own community. In other words, the community assignment for $v$ is correct. 

\begin{figure}[ht]
\centering
 \begin{tabular}{c | c}
    \includegraphics[width=.2\textwidth]{football_0} &
    \includegraphics[width=.2\textwidth]{football_30}
  \end{tabular}
  \caption{Football network with ground truth community shown in palette of rainbow colors. On the left is the original network while on the right is the same network with 30\% of the edges removed uniformly at random.}
  \label{foot}
\end{figure}

The value of permanence ranges from 1 (all neighbors form a cluster and are in the same community as the vertex) to -1 (all neighbors form a cluster and are in a different community than the vertex). Vertices in singleton communities have permanence zero. The permanence of a network is the average permanence of all its vertices. Therefore a network with more community-like structure will have higher permanence. For instance, the permanence of the node $v$ in Fig.~\ref{perm_toy} is equal to 0.12. 

Since it is vertex-centric, permanence can also be considered as a centrality metric, where vertices in tightly bound clusters are marked to be important. Nodes with high permanence indicate that their neighbors form cliques or near-cliques. While clustering coefficient can also provide this information, it considers the entire set of neighbors around a node $v$. In contrast, permanence uses a restricted set, consisting only those neighbors that are part of the same community as $v$. This difference between ordinary clustering coefficient and permanence is illustrated in Fig.~\ref{perm_toy}; consider the two nodes $x$ and $y$ both of which have exactly same clustering co-efficient but different values of permanence.  Therefore a high clustering coefficient does not indicate whether a vertex belongs to a community, whereas a high permanence means that the vertex belongs strongly within a community.

Permanence therefore provides a unique centrality value, that not only indicates the ranking of a vertex as per its importance, but also provides information about its position in a community. Because they belong to the core of communities,  high permanence vertices are very effective as seeds for broadcasting messages and also as good bases  for sampling.  Moreover, because these vertices belong to tightly connected clusters their overall rankings are less affected by the varying levels of noise in the system. Therefore message spreading and sampling using high permanence vertices is more resistant to noise within the network

Interestingly, the mean permanence over {\em all} the vertices is very sensitive to the effect of noise. In Fig.~\ref{foot}, we illustrate this phenomena for the structure of the well-known football network~\cite{girvan2002community} (see Section~\ref{setup} for description). The left network shows the community structures present in the original network (each community is represented by a different color), while the right network shows the structure when 30\% of the edges have been removed uniformly at random.  Note that the community labels for such moderate levels of perturbation to the network do not almost change.  Further, while the standard quality metrics like modularity, conductance and cut-ratio cannot signal the differences between the left and the right network, permanence is the only metric that signals this difference. While from left to right network, average permanence significantly declines from 0.266 to 0.071, the other metrics hardly change -- modularity changes from 0.553 to 0.557, conductance changes from 0.402 to 0.399 and cut-ratio changes from 0.039 to 0.028\footnote{Note the scale-size is 2, 2, 1, 1 for permanence, modularity, conductance and cut-ratio respectively.}. Thus mean permanence over the network is very appropriately sensitive to noise as compared to the other metrics.

%As we shall see in the later sections that the above quality of permanence makes it the only metric that is appropriately sensitive to noise (almost non-sensitive to low noise levels but highly sensitive larger noise levels).    


%Here we show how permanence can be used in applications beyond community detection, particularly its effectiveness under noise. We first compute permanence from the original community assignment of the network. For ease of explanation we assume that  the subset of neighbors covered by each vertex is such that these provide the highest clustering coefficient. Addition of an extra neighbor to the set will reduce the clustering coefficient, and removing a neighbor from the set, will either retain the same clustering co-efficient (if the rest of the neighbors form a clique) or become lower.  

%We then perturb the network using the different noise models described in ~\ref{ }. Because the noise level is low, we assume that the community assignment remains the same. Since all the models concern only removing edges, the permanence of the vertices, as well as the other metrics considered, will decrease ({\bf why other metrics decrease ?}).   

%We need to show that the value of permanence decreases (which improves sensitivity), but the ranking does not change, so the important vertices remain the same and useful for sampling and the spreading.  In contrast the other metrics change rank as well . What of random and Manhattan selection ?

%We show an illustrative example on football network as a toy model and  observe the effect of uniform noise on football network \cite{girvan2002community} at 30\% network perturbation in figure \ref{foot}. Using the ground community as the partition function on the network, we observe a decrease in  permanence  value  from  0.266  to  0.071  while  no significant change in  modularity(0.553 to 0.557), conductance(.402 to .399) or cut-ratio(0.039 to 0.028) ~\footnote{Note the scale-size is 2,2,1,1 for permanence, modularity, conductance and cut-ratio respectively.}. As evident from the example, the network structure is creating a re-organisation of the nodes and hence different community quality should be expected at different noise levels but modularity, cut-ratio and conductance are unable to capture the response. At higher noise levels, permanence is a composite metric that captures the quality of network structure(w.r.t perturbation of original network), community quality and possess sensitivity to noise levels which is missing from the metrics in existing literature.


%
%\subsection {Sensitivity to Noise.}  Need to explain why permanence decreases at a faster rate ($\frac{1}{n(n-1)}$), closeness ( max $\frac{(n-1)}{diameter^2}) others ?)
%
%
%\subsection {Robustness to Information Spreading.} 
%
%\subsection {Robustness to Sampling.} 

